Stability Via Adversarial Training of Neural Network Stochastic Control of Mean-Field Type

In this paper, we present an approach to neural network mean-field-type control and its stochastic stability analysis by means of adversarial inputs (aka adversarial attacks). This is a class of data-driven mean-field-type control where the distribution of the variables such as the system states and control inputs are incorporated into the problem. Besides, we present a methodology to validate the feasibility of the approximations of the solutions via neural networks and evaluate their stability. Moreover, we enhance the stability by enlarging the training set with adversarial inputs to obtain a more robust neural network. Finally, a worked-out example based on the linear-quadratic mean-field type control problem (LQ-MTC) is presented to illustrate our methodology.

==> MacrosMatematicas.tex <==
\makeatletter
\iflibroproyecto
%-------------------------Los elementos a,b,c,d---------------------------------------
\glossary(Elementos){$a$, $b$, $c$, $d$}{Elementos}%
%-------------------------Las variables w,x,y,z---------------------------------------
\glossary(Variables){$t$, $w$, $x$, $y$, $z$}{Variables}%
%-------------------------Los parámetros p,q,r,s--------------------------------------
\glossary(Parametros){$\alpha,\beta,\chi,\ldots$}{Parámetros}%
%-------------------------Variables índice y enteras--------------------------------------
\glossary(VariablesIndiceYEnteras){$i$, $j$, $k$, $l$, $m$, $n$}{Variables índice y enteras}%
\fi
%-------------------------El conjunto {a,b,c,d,...} de elementos a,b,c,d...-----------
\newcommand{\CtoEtos}[1]{\left\{\kern0.5pt #1\kern0.5pt\right\}}%
\iflibroproyecto
\glossary(ConjuntoElementos)%
{$\CtoEtos{a,b,c,\ldots}$}%
{Conjunto de los elementos $a$, $b$, $c$, $\ldots$}%
\fi
%-------------------------Conjunto de los a tales que P(a) {a|P}----------------------
\newcommand{\CtoPdadP}[2]{\CtoEtos{#1\mid #2}}%
\iflibroproyecto
\glossary(ConjuntoPropiedadP)%
{$\CtoPdadP{a}{P(a)}$}%
{Conjunto de los elementos $a$ con la propiedad $P(a)$}%
\fi
%-------------------------Conjuntos---------------------------------------------------
\newcommand{\Cto}[1]{\MakeUppercase{#1}}%
\iflibroproyecto
\glossary(Conjuntos){$\Cto{A}$, $\Cto{B}$, $\Cto{C}$, $\ldots$}{Conjuntos}%
\fi
%-------------------------Conjunto potencia-------------------------------------------
\newcommand{\CtoP}[1]{\mathcal{P}\left(\Cto{#1}\right)}%
\iflibroproyecto
\glossary(ConjuntoPotencia){$\CtoP{A}$}{Conjunto potencia de $\Cto{A}$}%
\fi
% ---------------------------Clase de Conjuntos (conjunto de conjuntos) ---------------------------
\newcommand{\ClsCto}[2]{\mathcal{#1}\left(\Cto{#2}\right)}%
\newcommand{\ClaseCto}[1]{\mathcal{#1}}%
\iflibroproyecto
\glossary(ClaseDeConjuntos)
{$\ClsCto{A}{B}$, $\ClaseCto{A}$}
{Clases de conjuntos (conjuntos de conjuntos)}%
\fi
%%\newcommand{\CtoPX}{\CtoP{\CtoX}}%
%  Conjunto potencia borroso
%%\newcommand{\CtoF}{\mathcal{F}\left(\CtoX\right)}%
% ---------------------------Complemento de un conjunto ---------------------------
\newcommand{\CCto}[1]{\overline{#1}}%
\iflibroproyecto
\glossary(ConjuntoComplemento){$\CCto{\Cto{A}}$}{Complemento del conjunto $\Cto{A}$}%
\fi
% ------------------Unión e intersección de conjuntos----------------------------------------------
\DeclareRobustCommand{\ICto}{\@ifstar{\bigcap}{\cap}}%
\DeclareRobustCommand{\UCto}{\@ifstar{\bigcup}{\cup}}%
\iflibroproyecto
\glossary(ConjuntosUnion)%
{$\UCto*\Cto{A}_i$, $\Cto{A}\UCto\Cto{B}$}%
{Unión de conjuntos}%
\glossary(ConjuntosInterseccion)%
{$\ICto*\Cto{A}_i$, $\Cto{A}\ICto\Cto{B}$}%
{Intersección de conjuntos}%
\fi
% ------------------Diferencia de conjuntos----------------------------------------------
\iflibroproyecto
\glossary(ConjuntoDiferencia)%
{$\Cto{A}-\Cto{B}$}%
{Conjunto diferencia formado por elementos que están en $\Cto{A}$ y no en $\Cto{B}$}%
\fi
%----------------------------Producto cartesiano de conjuntos--------------------------------------
\newcommand{\PCCto}{\times}%
\iflibroproyecto
\glossary(ProductoCartesiano)
{$\Cto{A}\PCCto\Cto{B}$}
{Producto cartesiano de los conjuntos $\Cto{A}$ y $\Cto{B}$}%
\glossary(ProductoCartesianoNVeces)
{$\Cto{A}^n$}
{Producto cartesiano $\Cto{A}\PCCto\Cto{A}\PCCto\cdots\PCCto\Cto{A}$ $n$ veces}%
\fi
%-----------------Conjunto de los números naturales, enteros y reales----------------------------
\newcommand{\CtoN}{\mathbb{N}}%
\newcommand{\CtoR}{\mathbb{R}}%
\newcommand{\CtoZ}{\mathbb{Z}}%
%\newcommand{\CtoQ}{\mathbb{Q}}%
\iflibroproyecto
\glossary(ConjuntoNaturalesEnterosReales)%
{$\CtoN$, $\CtoZ$, $\CtoR$}%
{Conjunto de naturales $\CtoEtos{1,2,\ldots}$,
enteros $\CtoEtos{\ldots,-1,0,1,\ldots}$ y reales}%
\fi
%------------------------------Conjunto Universal y vacío------------------------------------------
\newcommand{\CtoX}{\Cto{X}}%
\newcommand{\CtoV}{\emptyset}%
\iflibroproyecto
\glossary(ConjuntoUniversalVacio){$\CtoX$, $\CtoV$}{Conjunto universal y vacío}%
\fi
%---------------------------Pertenencia y no pertenencia al conjunto-------------------------------
%\in, \notin
\iflibroproyecto
\glossary(PertenenciaYNoPertenencia){$\in$, $\notin$}{Pertenencia y no pertenencia a un conjunto}%
\fi
%--------------------------Subconjunto y superconjunto---------------------------------------------
%\subseteq, \supseteq, \subset o \supset
\iflibroproyecto
\glossary(SubconjuntoYSuperconjunto)
{$\subseteq$, $\subset$,  $\supseteq$, $\supset$}
{Subconjunto, subconjunto propio, superconjunto, superconjunto propio}%
\fi
% Cardinalidad de un conjunto
%%\newcommand{\Card}[1]{\left|#1\right|}%
%------------------Relación binaria genérica. Subconjunto de AxB.-----------------------------------
\newcommand{\RBin}{R}%
\iflibroproyecto
\glossary(RelacionBinaria){$a\RBin b$}{Elemento $a$ relacionado con $b$ por medio de la relación binaria $\RBin$}%
\fi
%------------------Igualdad y no igualdad-----------------------------------------------------------
% =, \neq 
\iflibroproyecto
\glossary(IgualdadYNoIgualdad){$=$, $\neq$}{Igualdad y no igualdad}%
\fi
%---- Conectores lógicos ``y'', ``o'', ``no'', ``si entonces'', ``si y sólo si''.--------------------
\newcommand{\Cjc}{\text{y}}%
\newcommand{\Dyc}{\text{o}}%
\newcommand{\Neg}{\neg}%
\newcommand{\Imp}{\Rightarrow}%
\newcommand{\Coimp}{\Leftrightarrow}%
\iflibroproyecto
\glossary(ConectoresLogicos){$\Cjc$, $\Dyc$, $\Neg$, $\Imp$, $\Coimp$}
                            {Conectores lógicos ``y'', ``o'', ``no'', ``si entonces'', ``si y sólo si''}%
\fi
%  Cuantificador existencial
%\exists
%  Cuantificador universal
%\forall
%  Descriptor |
% |
% Equivalencia 
%\equiv--G
%------------------------------Relación de orden o desigualdades--------------------------------
% \leq, <, \geq ó >
\iflibroproyecto
\glossary(RelacionesDeOrdenMenorMayor)
{$\leq$, $<$, $\geq$, $>$}
{Relación de orden menor o igual, menor, mayor o igual, mayor}%
\fi
%------------------------------Símbolo de elementos 'incomparables'--------------------------------
\newcommand{\Incomp}{\mid\mid}%
\iflibroproyecto
\glossary(Incomparables){$a\Incomp b$}{Elementos $a$ y $b$ incomparables}%
\fi
% -----------------------------Supremo, ínfimo, máximo y mínimo--------------------------------------
% \max, \min \sup, \inf
\iflibroproyecto
\glossary(MaximoMinimoSupremoInfimo){$\max$, $\min$, $\sup$, $\inf$}{Máximo, mínimo, supremo e ínfimo}%
\fi
%----------------------------Operaciones conjunción y disyunción.-----------------------------
\DeclareRobustCommand{\OpCjc}{\@ifstar{\bigwedge}{\hspace{-0.5pt}\wedge\hspace{-0.5pt}}}%
\DeclareRobustCommand{\OpDyc}{\@ifstar{\bigvee}{\hspace{-0.5pt}\vee\hspace{-0.5pt}}}%
\iflibroproyecto
\glossary(OperacionConjuncionyDisyuncion)%
{$\OpDyc* a_i$, $\OpCjc* a_i$, $a\OpDyc b$, $a\OpCjc b$}{Disyunción y conjunción de elementos}%
\fi
%-------------------------------------Operación complemento------------------------------------------
\DeclareRobustCommand{\OpComp}[1]{#1^\prime}%
\DeclareRobustCommand{\OpCompinf}[1]{\OpComp{\underline{#1}}}%
\DeclareRobustCommand{\OpCompsup}[1]{\OpComp{\overline{#1}}}%
\iflibroproyecto
\glossary(OperacionComplemento){$\OpComp{a}$}{Complemento del elemento $a$}%
\fi
%-------------- El cero y la unidad de un conjunto --------------------------------------------------
\newcommand{\ElCero}{0}%
\newcommand{\LaUnidad}{1}%
\iflibroproyecto
\glossary(CeroYUnidad){$\ElCero$, $\LaUnidad$}{El cero y la unidad}%
\fi
%  Una manera de escribir retículo
%\newcommand{\Reticulo}[1]{\mathfrak{#1}}%--G
%-----Intervalos cerrado-cerrado, cerrado-abierto, abierto-cerrado, abierto-abierto ---------------
\newcommand{\IntCC}[1]{\left[#1\right]}%
\newcommand{\IntCA}[1]{\left[#1\right)}%
\newcommand{\IntAC}[1]{\left(#1\right]}%
\newcommand{\IntAA}[1]{\left(#1\right)}%
\iflibroproyecto
\glossary(Intervalos){$\IntCC{a,b}$, $\IntCA{a,b}$, $\IntAC{a,b}$, $\IntAA{a,b}$}{Intervalos}%
\fi
%-------------------------El Punto fijo del complemento--------------------------------------------
\newcommand{\ElPFC}{e_{c}}%
\iflibroproyecto
\glossary(PuntoFijo){$\ElPFC$}{Punto fijo del complemento}%
\fi
%  Isomorfismo
%%\newcommand{\Isomorfo}{\cong}%
%---------------------------Álgebras en notación A (versión *) ó (A,v,n,',0,1)--------------------
\DeclareRobustCommand{\Alg}{\@ifstar\Alg@i\Alg@ii}%
\DeclareRobustCommand{\Alg@i}[1]{\mathscr{\MakeUppercase{#1}}}%
\DeclareRobustCommand{\Alg@ii}[1]{\nTupla{#1;\OpDyc,\OpCjc,\OpComp{},\ElCero,\LaUnidad}}%
%\DeclareRobustCommand{\Alg@ii}[2][\ElCero,\LaUnidad]{\nTupla{#2\thinspace;\OpDyc,\OpCjc,\OpComp{},#1}}%
\DeclareRobustCommand{\AlgMorgan}[1][]{\Alg*{M}_{#1}}%--No está en glosario porque ya está \Alg.
\DeclareRobustCommand{\AlgKleene}[1][]{\Alg*{K}_{#1}}%--No está en glosario porque ya está \Alg.
\DeclareRobustCommand{\AlgBoole}[1][]{\Alg*{B}_{#1}}%--No está en glosario porque ya está \Alg.
\DeclareRobustCommand{\AlgFormulas}{\Alg*{F}}%--No está en glosario porque ya está \Alg.
\DeclareRobustCommand{\AlgTskLdbm}[1][]{\Alg*{T}_{#1}}%--No está en glosario porque ya está \Alg.
\iflibroproyecto
\glossary(Algebras){$\Alg*{A}$, $\Alg*{B}$, $\Alg*{C}$, $\ldots$}{Álgebras}%
\fi
%----------------------------Cociente--------------------------------------------------------------
\newcommand{\Coc}[2]{#1/#2}%
\iflibroproyecto
\glossary(Cociente){$\Coc{}{}$}{Cociente}%
\fi
%----------------------Una manera de escribir fórmula. f,h,g.-------------------------------------
\newcommand{\Frml}[1]{\MakeLowercase{#1}}%
\iflibroproyecto
\glossary(Formulas)%
{$\Frml{f}$, $\Frml{g}$, $\Frml{h}$, $\Frml{p}$, $\Frml{q}$, $\Frml{r}$, $\Frml{s}$}%
{Fórmulas o funciones definidas por fórmulas}%
\fi
%---------------------------Clase de equivalencia--------------------------------------------------
\newcommand{\ClsEquiv}[1]{\left[#1\right]}%
\iflibroproyecto
\glossary(ClaseEquivalencia){$\ClsEquiv{a}$}{Clase de equivalencia que contiene al elemento $a$}%
\fi
%---------------------------Fórmula f equivalente a g en el álgebra -------------------------------
\newcommand{\Fequiv}[1]{\equiv_{_{#1}}\hspace{-1.5pt}}%
\iflibroproyecto
\glossary(EquivalenciaFormula){$\Frml{f}\Fequiv{\Alg*{A}}\Frml{g}$}%
{Fórmulas $\Frml{f}$ y $\Frml{g}$ equivalentes sobre el álgebra $\Alg*{A}$}%
\fi
%  Operador de t-norma
%%\newcommand{\OpTnrm}{\@ifstar{\bigotimes}{\otimes}}%--G
%  Operador de T-conorma
%%\newcommand{\OpTcnrm}{\@ifstar{\bigoplus}{\oplus}}%--G
%  Operador complemento borroso
%%\newcommand{\OpCtoTTc}[1]{#1'}%
%---------------------------Operador de T-norma y T-conorma -------------------------------
\newcommand{\OpTn}{\bigtriangleup}%
\newcommand{\OpTc}{\bigtriangledown}%
\iflibroproyecto
\glossary(TnormaTconorma){$a\OpTc b$, $a\OpTn b$}%
{T-conorma y t-norma de los elementos $a$ y $b$}%
\fi
%---------------------------Operador de complemento difuso -------------------------------
\newcommand{\CompDif}{\@ifstar{\@SCompDif}{\@NSCompDif}}%
\newcommand{\@NSCompDif}[1]{\Lambda\left(#1\right)}%
\newcommand{\@SCompDif}{\Lambda}%
%--------------------- n-Tupla de elementos <x1,x2,...,xn>----------------------------------------
\DeclareRobustCommand{\nTupla}[1]{\left\langle #1\right\rangle}%
\iflibroproyecto
\glossary(Ntupla){$\nTupla{a_1,a_2,\ldots,a_n}$}{$n$-tupla de elementos}%
\fi
%  Vector de elementos [x1,x2,...,xn]
%%\newcommand{\VectorEtos}[1]{\left[#1\right]}%
%--------------------- Forma normal disyuntiva y conjuntiva -------------------------------------
\newcommand{\FND}[2]{\text{\normalfont D}_{_{#2}}(\Frml{#1})}%
\newcommand{\FNC}[2]{\text{\normalfont C}_{_{#2}}(\Frml{#1})}%
\iflibroproyecto
\glossary(FormasNormales)%
{$\FND{f}{\Alg*{A}}$, $\FNC{f}{\Alg*{A}}$}%
{Forma normal disyuntiva y conjuntiva de $\Frml{f}$ en el álgebra $\Alg*{A}$}%
\fi
%--------------------- Expansiones disyuntiva y conjuntiva -------------------------------------
\newcommand{\ED}[3][]{\text{\normalfont ED}_{_{#1}}^{#3}(\Frml{#2})}%
\newcommand{\EC}[3][]{\text{\normalfont EC}_{_{#1}}^{#3}(\Frml{#2})}%
\iflibroproyecto
\glossary(Expansiones)%
{$\ED[{\Alg*{A}}]{f}{x}$, $\EC[{\Alg*{A}}]{f}{x}$}%
{Expansión disyuntiva y conjuntiva de $\Frml{f}$ en $\Alg*{A}$ respecto a $x$}%
\fi
% ---------------------Transformaciones, mapeos, ... ---------------------------------------------
\iflibroproyecto
\glossary(Funciones){$\Phi$, $\Gamma$, $\Lambda$, $\Theta$,
                     $\Upsilon$, $\Omega$, $\Psi$}{Funciones o mapeos}%
\fi
% Composición entre transformaciones, mapeos, ...
\newcommand{\Comp}{\hspace{0.4pt}\circ\hspace{0.4pt}}%
% La flecha usada en los mapeos a-->b
\newcommand{\FlechaMap}{\hspace{-1pt}\mapsto\hspace{-1pt}}%--Esta macro no se considera que deba ir en el glosario
% ---------------------Caracter para indicar la no presencia de variable---------------------------
\newcommand{\NoVar}{\ifmmode\text{---}\else ---\fi}%
% -----Caracter para la separación de valores en el arreglo tabular propuesto----------------------
\newcommand{\CSep}{\thinspace\shortmid\thinspace}%
% -----Caracter para marcar los implicantes en el método de cubrimiento----------------------
\newcommand{\CMar}{\checkmark}%
% -----Caracter para cualquiera de las operaciones de disyunción o conjunción--------------------
\newcommand{\CDycCjc}{\star}%
% -----Operaciones de grupo --------------------
\newcommand{\OpBinGr}{\diamond}%
\newcommand{\OpUnGr}[1]{#1^{-1}}%
\newcommand{\IdGr}{e}%
% ----Macro para formatear los números de fila o columnas de tablas----------------------
\newcommand{\FNT}[1]{\textcircled{#1}}%{{\fboxsep1pt\framebox{#1}}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                             AMBIENTES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{demostracion}[1][Prueba]%
{\par\noindent\textbf{#1.}\nobreakspace}%
{\par}% Un ambiente para demostraciones
\iflibroproyecto
\newcounter{contejemplo}[chapter]%
\else
\newcounter{contejemplo}%
\fi
%\renewcommand{\thecontejemplo}{\arabic{chapter}.\arabic{contejemplo}}%
\newenvironment{ejemplo}{\vskip\baselineskip\par\noindent
\refstepcounter{contejemplo}%
\textbf{Ejemplo\nobreakspace\thecontejemplo}\nobreakspace}{\par}% Un ambiente para ejemplos
%\newenvironment{proof}%
%{\par\textbf{Prueba.}\nobreakspace}%
%{\par}% Un ambiente para Pruebas
\newtheorem{teorema}{Teorema}%                         Ambiente para teoremas 
%%\newtheorem{algoritmo}{Algoritmo}%                     Ambiente para algoritmos
\newtheorem{axioma}{Axioma}%                           Ambiente para axiomas
\newtheorem{corolario}{Corolario}%                     Ambiente para corolarios
\newtheorem{definicion}{Definici\'on}%                 Ambiente para definiciones
\newtheorem{lema}{Lema}%                               Ambiente para lemas
%%\newtheorem{proposicion}{Proposici\'on}%               Ambiente para propisiciones
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                             OTRAS DEFINICIONES MISCELANEAS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macro mara indicar el final de alguna cosa.
\newcommand{\Fin}{\nobreakspace\rule{0.5em}{0.5em}}%
% macro mara indicar el final de alguna cosa con espacio vertical agregado.
\newcommand{\FinEsp}[1][\baselineskip]{\Fin\vskip #1}%
